NeoHebbian Synapses to Accelerate Online Training of Neuromorphic Hardware

Neuromorphic systems that employ advanced synaptic learning rules, such as the three-factor learning rule, require synaptic devices of increased complexity. Herein, a novel neoHebbian artificial synapse utilizing ReRAM devices has been proposed and experimentally validated to meet this demand. This synapse features two distinct state variables: a neuron coupling weight and an "eligibility trace" that dictates synaptic weight updates. The coupling weight is encoded in the ReRAM conductance, while the "eligibility trace" is encoded in the local temperature of the ReRAM and is modulated by applying voltage pulses to a physically co-located resistive heating element. The utility of the proposed synapse has been investigated using two representative tasks: first, temporal signal classification using Recurrent Spiking Neural Networks (RSNNs) employing the e-prop algorithm, and second, Reinforcement Learning (RL) for path planning tasks in feedforward networks using a modified version of the same learning rule. System-level simulations, accounting for various device and system-level non-idealities, confirm that these synapses offer a robust solution for the fast, compact, and energy-efficient implementation of advanced learning rules in neuromorphic hardware.

==> tex_files/prior_works.tex <==
\section{Prior Works}
\label{prior_works}
One notable non-ideality in phase-change memory (PCM), namely resistance drift, has been leveraged for eligibility computation \cite{PCM_eprop}. Specifically, two PCM devices were employed within each synapse: one to implement the eligibility trace by utilizing the inherent resistance drift behavior of PCM, and the other to encode the coupling weight through its non-volatile conductance \cite{PCM_eprop}. However, this approach faces common challenges associated with PCM-based synapses, including significant day-scale drift toward the amorphous state, even in devices optimized for high retention, and an excessively abrupt reset transition. To address these issues, a differential pair synapse with a set-only programming scheme was proposed, though this design requires at least eight CMOS transistors per synapse, resulting in a large footprint and sparse synapse integration. In a separate study, the combined influence of electrical and optical stimuli on the switching behavior of non-volatile Ag/GeSe$_{3}$/Ag memristive devices was explored \cite{Sarwat2021ChalcogenideOF}. For example, when an electrical pulse was applied to an illuminated device, it spontaneously transitioned to a conducting state. In contrast, no resistive switching occurred if the device was illuminated without a voltage stimulus, or if a sub-threshold electrical stimulus was applied in dark conditions. Utilizing this behavior, the authors demonstrated the implementation of a three-factor learning rule. While these devices hold promise for high-density integration, energy consumption could be a limiting factor, with total energy consumption primarily driven by optical power, typically within the milliwatt range \cite{Sarwat2021ChalcogenideOF}. 
Other research has focused on using PCM devices solely for storing coupling weights, employing high-precision computational units for eligibility trace computation \cite{Bohnstingl_AICAD_2022, ortner2024learning}, or utilizing mixed-signal analog/digital neuromorphic circuits \cite{Charlotte_ISSCC_2022}. However, both approaches face challenges related to transistor scaling, especially for large-scale network implementations. Consequently, there remains significant scope for developing neo-Hebbian synapses that harness memristor physical dynamics for the hardware implementation of advanced learning rules.

